Planning Multiple Epidemic Interventions with Reinforcement Learning

Combating an epidemic entails finding a plan that describes when and how to apply different interventions, such as mask-wearing mandates, vaccinations, school or workplace closures. An optimal plan will curb an epidemic with minimal loss of life, disease burden, and economic cost. Finding an optimal plan is an intractable computational problem in realistic settings. Policy-makers, however, would greatly benefit from tools that can efficiently search for plans that minimize disease and economic costs especially when considering multiple possible interventions over a continuous and complex action space given a continuous and equally complex state space. We formulate this problem as a Markov decision process. Our formulation is unique in its ability to represent multiple continuous interventions over any disease model defined by ordinary differential equations. We illustrate how to effectively apply state-of-the-art actor-critic reinforcement learning algorithms (PPO and SAC) to search for plans that minimize overall costs. We empirically evaluate the learning performance of these algorithms and compare their performance to hand-crafted baselines that mimic plans constructed by policy-makers. Our method outperforms baselines. Our work confirms the viability of a computational approach to support policy-makers

==> 02-background.tex <==



==> tables/actionspace-table-old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[tb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ll|lcl|cc|ccc@{}}
\toprule
 &
   &
  \multicolumn{3}{c}{\textbf{Control Parameter}} &
  \multicolumn{2}{l}{\textbf{Action Spaces}} &
  \multicolumn{3}{c}{\textbf{Baseline Policies}} \\ \midrule
 &
  \textbf{Intervention} &
  \textbf{} &
  \textbf{Range} &
  \textbf{Description of control parameter} &
  \textbf{A} &
  \textbf{B} &
  \textbf{Aggressive} &
  \textbf{Lax} &
  \textbf{Random} \\
1 &
  Mask-wearing &
  \begin{tabular}[c]{@{}l@{}}Compliance \\ Degree\end{tabular} &
  [0, 1] &
  \begin{tabular}[c]{@{}l@{}}Affects the transition from S to I by modifying the transmissibility \\ $\beta$ rate. Higher compliance reduces the transmissibility rate.\end{tabular} &
  Y &
  Y &
  0.8 &
  1 &
  $\sim U(0,1)$ \\
2 &
  Vaccination &
  \begin{tabular}[c]{@{}l@{}}Administration \\ Rate\end{tabular} &
  [0, 1] &
  \begin{tabular}[c]{@{}l@{}}Affects the proportion of individuals that move from S to R in SIR, \\ S to V1 in SIRV and S to V in COVID-19. A higher rate means that a \\ higher proportion of the susceptible population gets vaccinated.\end{tabular} &
  Y &
  Y &
  85\% population in 9 months &
  70\% population in 12 months &
  $\sim U(0,1)$ \\
3 &
  School closure &
  \begin{tabular}[c]{@{}l@{}}Remote learning \\ proportion\end{tabular} &
  [0, 1] &
  \begin{tabular}[c]{@{}l@{}}Higher proportions lower infectious interactions within school \\ facilities; 0 means no remote learning/school closure.\end{tabular} &
   &
  Y &
  \begin{tabular}[c]{@{}c@{}}if $t \in [0, 120]$ then 1, \\ 0.5 otherwise;\end{tabular} &
  0 &
  $\sim U(0,1)$ \\
4 &
  Workplace closure &
  \begin{tabular}[c]{@{}l@{}}Remote working \\ proportion\end{tabular} &
  [0, 1] &
  \begin{tabular}[c]{@{}l@{}}Higher proportions lower infectious interactions within workplace \\ facilities; 0 means no workplace closures.\end{tabular} &
   &
  Y &
  \begin{tabular}[c]{@{}c@{}}if $t \in [0, 120]$ then 1, \\ 0.5 otherwise;\end{tabular} &
  0 &
  $\sim U(0,1)$\\
  \bottomrule
\end{tabular}%
}
\caption{The four interventions under consideration. As the complexity of the action space increases from A to B, more interventions are considered as indicated. The Aggressive and the Lax baseline plans have pre-defined control parameter settings for the interventions, while the values for the Random baseline control parameters are sampled uniformly at random from the parameter's range.}

\label{tab:interventions}
\end{table*}

==> tables/bestperformance-table.tex <==
\begin{table}[htb]
\begin{tabular}{ |p{1.5cm}||p{2.5cm}|p{2.5cm}|}
 \hline
 Algorithms & \textbf{SIR-A} & \textbf{SIR-B}\\
\hline
Lax& $-1.04 \times 10^{8}$&$-1.04 \times 10^{8}$\\
\hline
Aggressive& $-1.36 \times 10^{8}$&$-1.58 \times 10^{9}$\\
\hline
Random& $-1.10 \times 10^{8} \pm 2.00 \times 10^{7}$&$-7.45 \times 10^{8} \pm 4.66 \times 10^{7}$\\
\hline
PPO& $-4.33 \times 10^{7} \pm 2.02 \times 10^{5}$&$-4.25 \times 10^{7} \pm 3.09 \times 10^{5}$\\
  \hline
SAC& $-9.24 \times 10^{7} \pm 5.87 \times 10^{5}$&$-7.58 \times 10^{8} \pm 4.46 \times 10^{6}$\\
  \hline
 \hline
  & \textbf{SIRV-A} & \textbf{SIRV-B}\\
\hline
Lax& $-1.22 \times 10^{8}$&$-1.16 \times 10^{8}$\\
\hline
Aggressive& $-1.66 \times 10^{8}$&$-1.58 \times 10^{9}$\\
\hline
Random& $-2.80 \times 10^{9} \pm 1.05 \times 10^{9}$&$-8.12 \times 10^{8} \pm 6.18 \times 10^{7}$\\
\hline
PPO& $-8.25 \times 10^{7} \pm 2.11 \times 10^{5}$&$-7.91 \times 10^{7} \pm 1.81 \times 10^{5}$\\
  \hline
SAC& $-1.28 \times 10^{9} \pm 1.28 \times 10^{8}$&$-7.87 \times 10^{8} \pm 6.76 \times 10^{6}$\\
  \hline
 \hline
  & \textbf{Covid19-A} & \textbf{Covid19-B}\\
\hline
Lax& $-1.68 \times 10^{8}$&$-1.67 \times 10^{8}$\\
\hline
Aggressive& $-1.40 \times 10^{8}$&$-7.43 \times 10^{8}$\\
\hline
Random& $-9.05 \times 10^{8} \pm 2.91 \times 10^{8}$&$-4.15 \times 10^{8} \pm 2.05 \times 10^{7}$\\
\hline
PPO& $-4.53 \times 10^{7} \pm 3.40 \times 10^{4}$&$-5.51 \times 10^{7} \pm 9.87 \times 10^{6}$\\
  \hline
SAC& $-3.34 \times 10^{8} \pm 7.04 \times 10^{6}$&$-4.02 \times 10^{8} \pm 4.80 \times 10^{6}$\\
  \hline
\end{tabular}
\caption{Mean and standard deviation of the best performance of each algorithm across different random seeds.}

\label{table:best}
\end{table}

==> tables/hyperparameter-table.tex <==
\begin{table*}[htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}[t]{llcc}
\toprule
\textbf{SAC Hyperparameter} & 
\multicolumn{1}{c}{\textbf{Description}}
& \textbf{Grid-search values}  
& \textbf{Chosen value} \\ 
\midrule

Reward scale                                    
 & \begin{tabular}[t]{@{}l@{}}This is the multiplicative scaling applied after the normalized rewards. \\ It is equivalent to inverse of entropy regularization coefficient\end{tabular} 
 & \begin{tabular}[t]{@{}c@{}}{[}1, 10, 100, \\1000{]}  \end{tabular}      
 & 100                   \\[0.15cm]

Learning rate                                   
& \begin{tabular}[t]{@{}l@{}}Learning rate for Adam optimizer, the same learning rate \\ will be used for all networks (Q-Values, Actor and Value function)\end{tabular}                
& \begin{tabular}[t]{@{}c@{}}{[}0.003, 0.0003,\\ 0.00003{]} \end{tabular}  
& 0.0003                \\[0.15cm]

Training frequency                             
& The number of simulation timesteps to update the model
& {[}5, 25, 125{]}             
& 5                     \\[0.15cm]

Learning starts                                 
& \begin{tabular}[t]{@{}l@{}}How many steps of the model to collect transitions for before \\ learning starts\end{tabular} 
& \begin{tabular}[t]{@{}c@{}}{[}1000, 5000, \\10000{]} \end{tabular}     
& 1000                  \\[0.15cm]

Batch size
& Minibatch size for each gradient update   
&                              
& 256                   \\[0.15cm]


Tau                                             
& The soft update coefficient (``Polyak update", between 0 and 1)            &                             
& 0.005                 \\[0.15cm]

Gamma                                           
& The discount factor                                                        &                             
& 0.99                  \\[0.15cm]

Buffer size                                     
& Size of the replay buffer 
&
& 1000000               \\[0.15cm]


Gradient steps                                  
& How many gradient steps to do after each rollout     
&                              
& 1                     
\\ \midrule

\textbf{PPO Hyperparameter}
& 
&
&
\\ \midrule

Learning rate                                   
& The learning rate of the optimizer
& 
&0.0003\\[0.15cm]

Num steps                                       
& The number of steps to run in each environment per policy rollout   
& 
&2048\\[0.15cm]

Gamma                                           
& The discount factor
& 
&0.99\\[0.15cm]

Gae Lambda
& The lambda for the general advantage estimation                            & 
&0.95\\[0.15cm]

Num minibatches 
& The number of mini-batches                                                 & 
&32\\[0.15cm]

Update epochs 
& The K epochs to update the policy                                          &
&10\\[0.15cm]

Clip coefficient
& The surrogate clipping coefficient
&
&0.2\\[0.15cm]

Entropy coefficient
& Coefficient of the entropy
&
&0.0\\[0.15cm]

Vf coefficient
& Coefficient of the value function
&
&0.5\\[0.15cm]


Max grad norm
& The maximum norm for the gradient clipping                                 
&
&0.5\\
\bottomrule
\end{tabular}
}
\caption{The hyperparameter settings for SAC and PPO.}
\label{tab:hyperparameter}
\end{table*}
